Anaysis of the validity of P2D models for solid-state batteries in a large parameter range

Simulation models are nowadays indispensable to efficiently assess or optimize novel battery cell concepts during the development process. Electro-chemo-mechano models are widely used to investigate solid-state batteries during cycling and allow the prediction of the dependence of design parameters like material properties, geometric properties, or operating conditions on output quantities like the state of charge. One possibility of classification of these physics-based models is their level of geometric resolution, including three-dimensionally resolved models and geometrically homogenized models, known as Doyle-Fuller-Newman or pseudo two-dimensional models. Within this study, the advantages and drawbacks of these two types of models are identified within a wide range of the design parameter values. Therefore, the sensitivity of an output quantity of the models on one or a combination of parameters is compared. In particular, the global sensitivity, i.e., the sensitivity in a wide range of parameter values, is computed by using the Sobol indices as a measure. Furthermore, the local sensitivity of the difference in the output quantities of both models is evaluated to identify regions of parameter values in which they contain significant deviations. Finally, remarks on the potential interplay between both models to obtain fast and reliable results are given.

==> chapters/sobol.tex <==
\section{Quantification of the global sensitivity by Sobol indices}
\label{sec:sobol_indices}
Sobol indices quantify the influence of one parameter or a combination of parameters on an output quantity of a model or an experiment. The set of~$n$ input parameters is denoted by~$~\vec{X}$, and the output quantity by~$Y(\vec{X})$. The expectation value~$E(Y)$ and the variance~$V(Y)$ of the output quantity are computed for different combinations of the input parameters. The Sobol indices of first-order are defined by the variance of the expectation value when keeping the parameter~$X_i$ fixed, i.e., $V_i = V(E(Y|X_i))$. Normalizing this value by the variance of the entire input parameter range results in the first-order Sobol index
\begin{equation}
    S_i = \frac{V(E(Y|X_i))}{V(Y)}.
\end{equation}
In a similar way, higher-order Sobol indices are defined. Then, the number of parameters that equal the order of the index is simultaneously fixed. The values of the higher order Sobol indices are then corrected by the values of the lower orders for these parameters, e.g., for the second-order Sobol index
\begin{equation}
    S_{ij} = \frac{V(E(Y|X_i,X_j))}{V(Y)} - S_i - S_j.
\end{equation}
By this definition, all Sobol indices up to $n$-th order sum up to one. \\
The total-order Sobol index is defined as the normalized expectation value of the variance if all parameters except one are fixed. It is defined by
\begin{equation}
    S^\text{t}_i = \frac{E(V(Y|X \backslash X_i))}{V(Y)}.
\end{equation}
By definition, all Sobol indices up to $n$-th order related to the parameter~$X_i$ sum up to~$S^\text{t}_i$. In particular, it tells if a parameter has an influence at all either isolated or in combination with other parameters. \\
The numerical computation of the Sobol indices might become costly, as it requires computing the conditional expectation value and afterwards its variance. Typically, the computation of the expectation value and the variance is performed using Monte-Carlo integration~\cite{Sobol2001}. The computational costs for this nested operation to compute the first- and total-order Sobol indices scale with~$\mathcal{O}(M^2)$, where~$M$ is the number of Monte-Carlo samples that is recommended to be sufficiently large (c.f.~\cite{Wirthl2023}). The number of model evaluations can be reduced to~$M(2D+2)$ evaluations, with the number of input parameters~$D$ using an approach as done in~\cite{Saltelli2010}.
